Is Large Language Model Good at Database Knob Tuning? A Comprehensive Experimental Evaluation

Knob tuning plays a crucial role in optimizing databases by adjusting knobs to enhance database performance. However, traditional tuning methods often follow a Try-Collect-Adjust approach, proving inefficient and database-specific. Moreover, these methods are often opaque, making it challenging for DBAs to grasp the underlying decision-making process. The emergence of large language models (LLMs) like GPT-4 and Claude-3 has excelled in complex natural language tasks, yet their potential in database knob tuning remains largely unexplored. This study harnesses LLMs as experienced DBAs for knob-tuning tasks with carefully designed prompts. We identify three key subtasks in the tuning system: knob pruning, model initialization, and knob recommendation, proposing LLM-driven solutions to replace conventional methods for each subtask. We conduct extensive experiments to compare LLM-driven approaches against traditional methods across the subtasks to evaluate LLMs' efficacy in the knob tuning domain. Furthermore, we explore the adaptability of LLM-based solutions in diverse evaluation settings, encompassing new benchmarks, database engines, and hardware environments. Our findings reveal that LLMs not only match or surpass traditional methods but also exhibit notable interpretability by generating responses in a coherent ``chain-of-thought'' manner. We further observe that LLMs exhibit remarkable generalizability through simple adjustments in prompts, eliminating the necessity for additional training or extensive code modifications. Drawing insights from our experimental findings, we identify several opportunities for future research aimed at advancing the utilization of LLMs in the realm of database management.

==> LLM.tex <==
\section{Performance Comparison on different LLMs(Q4)}
ChatGPT has garnered significant interest from the AI community since its release due to its exceptional ability to communicate with humans. Notably, ChatGPT [LLM\_survey\_Chinese 84] and GPT-4 [45] have significantly enhanced existing capabilities and are considered milestones in the field. Our work primarily revolves around these two models. However, with the continuous development of large language model (LLM) technology, a variety of LLMs have emerged in the market, such as PaLM [huangXM 6] , LLaMa [34], etc. How do these large language models perform in tuning tasks compared to ChatGPT? How should we choose the appropriate LLM for knob tuning tasks? To explore these questions, this section will compare the performance of different LLMs in knob tuning.

\subsection{Setup}

\input{tables/llms}
In this section, the LLMs we use include ChatGPT-3.5, ChatGPT-4, Kimi, LLaMA, among others. From a scale perspective, these models can be divided into two categories: those with tens of billions of parameters and those with hundreds of billions of parameters. From a usage perspective, they can be categorized as either publicly accessible or closed-source. Detailed information about each model is shown in \autoref{tab:llms}.

\subsection{Result}
The test results are shown in \autoref{fig:llms}. It can be seen that GPT-4 achieved the best results among all methods. This is not surprisingly cause GPT-4 has a larger scale, more comprehensive corpus, stronger ability to solve complex tasks, and shows significant performance improvement in many evaluation tasks compared to other models. A recent study [LLM \_survey-C 40] investigate the performance of GPT-4 by conducting qualitative tests on human generated problems
The tests in cover various difficult tasks, and the results show that GPT-4 has better performance than previous GPT models. By comparing and analyzing the performance of other LLMs, it is not difficult to find that (1) the performance of closed source LLMs far exceeds of open source LLMs, (2) the larger the number of parameters in LLM, the better their performance.

\iffalse
测试结果如图X所示。可以看出GPT-4在所有方法中取得了最好的效果。这并不出乎我们的意料,相比其他模型,GPT-4有着更大的规模、更充分的语料,在解决复杂任务方面具有更强的能力,在许 多评估任务上展现出大幅度的性能提升。最近的一项研究 [LLM\_survey-C 40] 通过开展人类生成问题的定性测试来研究 GPT-4 的性能,其
中的测试涵盖了各种困难任务,结果显示 GPT-4 具有比之前
的 GPT 模型如 ChatGPT 更出色的性能。而通过对比分析其它LLM的表现,我们不难发现,总体来看1、闭源LLM的性能远超开源,2、在同类大模型中,参数量越大其表现越好。
\fi

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/LLMs.png}
    \caption{Architecture of Configuration Tuning System} 
    \label{fig:llms}
\end{figure}

The main reasons for the previous pattern include (1) corpus, (2)training and (3)fine-tuning. In terms of corpus, the quantity and quality of corpus used during pretraining have a significant impact on performance. Chinchilla [survey 33] indicates that many existing LLMs suffer from suboptimal training due to a lack of sufficient pretraining data. When pre training low-quality corpora, such as noisy, harmful, and repetitive data, it may also damage the performance of the model [survey 59, 158, 160, 163]. Compared to open source models, closed source models such as GPT often have more abundant and high-quality corpus. In terms of training, most closed source models are released by enterprises such as OpenAI, which have sufficient time, hardware and other resources to fully train the model and unleash its potential. In addition, large enterprises also have more sufficient trial and error costs and the ability to explore different model architectures. In terms of fine-tuning, high-quality human feedback is crucial for aligning LLM with human preferences and values, helping LLM to further adapt its universal ability to solve various tasks to specific goals, such as the database parameter tuning that this article focuses on. And these high-quality human feedback also require human and financial support, which is exactly the advantage of enterprises.

The latter rule is easier to understand, as researchers in the President train Langauge Model (PLM) stage have found that extending PLM (such as expanding model size or data size) usually improves the model performance of downstream tasks (i.e. following the extension rule [30]). Many studies have explored performance limits by training increasingly large PLMs, such as GPT-3 with 175 billion parameters and PaLM with 540 billion parameters.

\iffalse
对于前一个规律,其主要原因包括1、语料 2、训练 3、微调。语料方面,预训练时用到的语料的数量和质量都对性能有着重要影响。Chinchilla [survey 33] 表明,许多现有的LLM 由于缺乏充足的预训练数据而遭受次优训练的问题。而对低质量的语料库进行预训练时,例如噪声、有害和重复的数据,同样可能会损害模型的性能 [survey 59, 158, 160, 163]。相较开源模型来说,GPT等闭源模型往往有着更充足且高质量的语料。训练方面,闭源模型大多由OpenAI等企业发布,其有着充足的时间、硬件等资源,充分训练模型,发挥其潜能。此外,大型企业也有着更充足的试错成本,有能力探索不同的模型架构架构。微调方面,高质量的人类反馈对于将 LLM 向人类的偏好和价值观对齐非常重要,帮助LLM将 可以获得解决各种任务的通用能力进一步适配(adapting)到特定的目标中,如本文所关心的数据库参数调优。而这些高质量的人类反馈同样需要人力与资金支持,这正是企业的优势所在。
后一个规律则更容易理解,在PLM(President-train Langauge Model)阶段研究人员就已经发现,扩展 PLM(例如扩展模型大小或数据大小)通常会提高下游任务的模型性能(即遵循扩展法则 [30])。许多研究通过训练越来越大的 PLM(例如 1750 亿参数的 GPT-3 和 5400 亿参数的 PaLM)来探索性能极限。
\fi

\iffalse
其中ChatGPT由于具备与人类进行交流的出色能力, 自从发布以来便引发了 AI 社区的极大兴趣。特别是ChatGPT[LLM\_survey\_Chinese 84]和GPT-4[45],这两个模型大大提升了现有的能力,有着里程碑式的意义。我们的工作也大多围绕这两个模型展开。但近年来随着大语言模型相关技术的不断发展,市面上各类LLM层出不穷,如PaLM [huangXM 6 ], and LLaMa [ 34]等等。与ChatGPT相比,这些大预言模型在调优任务上表现如何？如何选择合适的LLM作为参数调优任务的基础？为了探究这些问题,本节我们将采用不同的大语言模型进行参数调优,并对比其性能。
在本节中,我们所使用LLM模型包括ChatGPT-3.5,ChatGPT-4,Kimi,LLaMA等等。从规模上来看,可将其分为百亿参数量级别和千亿参数量级别两类；从使用的角度来看,可将其分为可公开获取和闭源两种。各模型的详细信息如表X所示。
\fi

==> overview.tex <==
\section{Knob Tuning Overview}




The overall workflow of database knob tuning is illustrated in \autoref{fig:overview}. The left part shows the target DBMS and the replayed workload. The right part represents the tuning server deployed in the backend tuning cluster. The tuning system can be divided into three parts: knob selection , knob recommendation , and knowledge transfer .

The configuration optimization module functions iteratively, (1) The controller replays the workload to conduct stress testing. (2) After the stress testing finishes, the performance statistics are uploaded to the data repository and used for updating the model in the configuration optimizer. Optionally, the knowledge transfer module can speed up the optimization with historical observations. (3) The optimizer generates a promising configuration over the pruned configuration space, and the configuration is applied to the target DBMS through the controller. The above procedures repeat until the model of the optimizer converges or stop conditions are reached (e.g., budget limits). Next We present each of these three important components.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/image.png}
%     \caption{Architecture of Configuration Tuning System} 
%     \label{fig:overview}
% \end{figure}
\vpara{Knob selection}  Database systems contain hundreds of knobs that (1) have various effects on tuning performance (e.g., working memory size is vital to memory-intensive queries, maximum IO concurrency is vital to IO-intensive queries), and (2) correlations between knobs can significantly affect the performance (e.g., the maximum number
of user connections is limited by the allocated resources).  But only a subset actually affect the DBMS’s performance. Thus, reducing the number of knobs limits the total number of possible DBMS configurations that must be considered. Knob selection determines which knobs to adjust. 

Traditional knob selection methods rely on DBAs to select important or suitable knobs. However, this leads to a huge burden for DBAs to handle hundreds of knobs. Thus, some tuning methods propose a knob selection module in their framework, i.e., empirical-based method and ranking-based method. Empirical-based knob selection requires humans (e.g., database users, DBAs) to select knobs based on limited tuning documents or empirical experience.  However, it is hard for humans to identify the complex correlations between various knobs (e.g., the maximum values of some knobs may rely on other knobs). Ranking-based methods sort the knobs based on their impact on the database performance and select the knobs with large impacts [22], [66], [76]. Ranking-based knob selection methods require to find the relations between the knobs and performance. However, since there are hundreds of knobs, only a small number of knobs are involved in knob selection, which may introduce bias.

%There are two main challenges for knob selection: selecting important knobs and selecting suitable knobs. The former means that only those knobs have a major impact on performance should be considered in the tuning process. For example, many methods [tuning survey 9], [19], [39], [74], [79] identify important knobs before actual knob tuning to reduce the tuning overhead. The latter means selecting knobs that are suitable for different scenarios. Traditional knob selection methods include empirical-based method, ranking-based method, and learning-based method.

\vpara{Knob Recommendation} 
knob recommendation employs algorithms to suggest specific parameter values. We can formalize the knob tuning problem into an optimization problem, which given a workload and a suite of adjustable knobs,
select the optimal knob settings under predefined objectives and constraints (e.g., maximizing the throughput within
limited memory space). Traditional tuning methods rely on DBAs to manually tune the knobs. However, these manual tuning methods are timeconsuming and highly dependent on the DBA’s experience. Many tuning methods are proposed to address these limitations. Researchers propose intelligent tuning to combine machine learning methods. We categorize existing studies into four categories: (1) heuristic tuning methods, (2) Bayesian optimizationbased tuning methods, (3) deep learning-based tuning methods, and (4) reinforcement learning-based tuning methods.
As the knob tuning problem is NP-hard, one tuning method cannot perform well under all the scenarios (e.g., heuristic methods achieve low tuning overhead; while learning-based methods can utilize historical tuning experience and optimize the performance). 

\vpara{Knowledge Transfer}
In real scenarios, the workloads could dynamically change. For example, the workload pressure may change significantly over time (morning to evening, weekday to weekend, or workday to holiday). Generally, a single knob setting cannot be optimal for all tuning tasks, because the knob-performance relations and tuning requirements may change on the new scenarios, and the tuning models trained on historical tuning tasks cannot be directly used (fine-tune or retrain new models from scratch). Hence, it is vital but challenging to adapt to workload changes or new tuning tasks in real scenarios [26], [52], [92]. Most existing machine learning models (e.g., reinforcement learning) cannot directly recommend high-quality knob settings for new tuning tasks. In other words, whenever the workload changes, these methods need to train from scratch, which is time-consuming and wastes many system resources. Besides, new tuning features make it even harder to adapt to new scenarios. To adapt to dynamic workloads, transfer techniques aim to improve tuning efficiency by migrating the knowledge learned from historical tuning tasks to new tuning tasks. Currently, three transfer techniques have been proposed in knob tuning [79], [52], [26], [88], [26], [10], including workload mapping, fine-tune, and model ensemble.
%With well-learned tuning models on historical tasks, transferring those models to new tuning tasks (e.g., tuning for workloads with completely new operators, datasets, or even hardware environments). Moreover, it is vital to achieve practical learned tuning methods in real scenarios. Thus, transfer techniques are proposed to support dynamic scenarios at different levels (e.g., various workloads and databases). 
%Currently, three transfer techniques have been proposed in knob tuning [tuning survey 79], [52], [26], [88], [26], [10], including workload mapping, learned workload embedding, and model ensemble. These transfer techniques could enhance the adaptivity of tuning methods for dynamic workloads.




==> prompt.tex <==
\section{Performance Comparison on different prompts}
\label{sec: prompts}
In this section, we primarily focus on the impact of different prompts on the LLM tuning.  Prompts have emerged as a crucial technique for harnessing the potential of large language models. However, crafting effective prompts is challenging and demands extensive trial and error, as these models are highly responsive to variations in prompts. This sensitivity is particularly pronounced in knob tuning tasks, which require precise handling of numerical values.


Prompts generally consist of instructions, questions, input data, and examples. In practice, to elicit a desired response from an AI model, a prompt must contain either instructions or questions, with other elements being optional. To determine the most effective prompt construction for tuning tasks, we systematically explore various configurations of each component and experimentally evaluate their respective tuning performances. 

Knob recommendation is the most core component in the whole tuning process, which directly affects the tuning effect, so in this section our experiments mainly focus on it. According to the results of \autoref{sec:recommend result}, Claude3 has the best effect in knob recommendation task, so we choose it as the base model.

% \subsection{Instructions and Questions}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/CoT.png}
%     \caption{Two different approaches to prompting. (1)Directly recommend specific values. (2)First select the adjustment direction, then determine the magnitude of change.} 
%     \label{fig:CoT}
% \end{figure}

As shown in \autoref{fig:CoT}, There are two representations of the tuning problem, (1) direct tuning and (2) incremental tuning. The former requires the LLM to directly provide specific values for each knob, while the latter requires the LLM to inform the user of the tuning direction (increase or decrease) and then determine the magnitude of change. Mathematically, these two approaches are essentially equivalent. Traditional algorithms typically prefer direct tuning because, whether using BO-based methods or RL-based methods, the focus is on the performance of the database under specific configurations (i.e., a sampling point in the parameter space) without considering the state before the transition. However, for LLMs, incremental tuning transforms the implicit reasoning steps of LLMs into an explicit, guided two-step sequence, namely Chain of Thought (CoT). 

%\input{tables/prompt_question}

 Contrary to our expectations, CoT does not enhance performance in experiment, it has an adverse effect instead. Observations indicate that after applying CoT, the database performance even fall below the default configuration. More critically, incorrect configurations emerge during the recommendation process. For example, the knob \textit{innodb\_compression\_failure\_threshold\_pct} controls the threshold for table compression failure rate in MySQL. When this threshold is exceeded, the database increases the reserved space in compressed pages. Its value range is an integer between 0 and 100, but LLM set it to 7.5 when tuning in the CoT format. Another knob, \textit{innodb\_spin\_wait\_delay}, controls the spin wait delay time in the storage engine, measured in microseconds. The LLM set this to a negative number when tuning in the CoT format. These errors are serious and can prevent the database from starting properly, which is unacceptable during tuning. We found that these issues occurred in the second step of CoT. In other words, after applying CoT, the LLM correctly identified the tuning direction (whether to increase or decrease) but struggled to estimate the magnitude of the adjustment. We consider this is due to the LLM's insensitivity to numbers. It remains fundamentally a language model, and numbers are merely strings to it. In direct tuning, knobs' names and values are provided sequentially, maintaining a close contextual relationship. However, in incremental tuning the process is split into two steps, and the LLM must also relate to the current knob values to determine the appropriate adjustment, significantly increasing the difficulty of generating numbers. Therefore, our recommendation is to construct prompts in a direct generation format when using LLM for knob tuning.

\subsection{Input Data}

As previously mentioned, input data is an optional component for prompts, and this applies to tuning tasks as well.  The optional information that can be included in the prompt for the LLM consists of (1) description of the tuning task (explaining knob tuning, the relationship between database configurations, inner metrics, and performance), (2) details about knobs and features (which knobs and inner metrics are used, and the roles of each knob and inner metric) and (3) relevant information about the current tuning task (such as hardware environment, workload, etc.).

Providing these information can assist  LLM in better understanding the tuning task. However, some of these information may already be familiar to the LLM from its training data and may not need to be repeated. Moreover, overly detailed information can potentially interfere with the LLM's judgment to some extent and affect generation efficiency. Therefore, it is important to experimentally identify the most useful input data.

\input{tables/prompt_input}

The results are shown in \autoref{tab:prompt_input}. We found that without providing any additional information, LLM is unable to independently complete the tuning task, i.e., it cannot provide specific values. This is mainly because knob tuning tasks are relatively broad, and different hardware and database kernels significantly impact tuning, making input information such as knob information essential . This also explains why, when providing only one type of input, it is crucial to include current environment information for LLM . In such cases, LLM also achieves good tuning results. 
When two types of inputs are provided, the importance of current environment information is further confirmed: when both environment information and task description are present, the tuning results are nearly as good as when all three types of inputs are provided. Conversely, when current environment information is excluded, the tuning effectiveness with task description and knob information is even worse than with environment information alone. Strangely, providing both task description and current environment information to the LLM leads to confusion, resulting in unusual knob selections and values, including some completely unrelated knobs. Consequently, the tuning effectiveness is very limited, only slightly better than the default configuration. Our analysis suggests that this is mainly because the task description emphasizes the important relationship between knobs, inner metrics, and performance, but without specific explanations (i.e., knob information), it confuses the LLM, preventing it from making relatively general configuration recommendations based solely on the current environment.

In summary, we believe that when using LLM for knob tuning, the importance of input data, from most to least important, is as follows: current environment, konb information, and task description. If efficiency is a priority or there is a lack of informtion of knobs, it is sufficient to provide only current environment information, including hardware environment, database kernel, and workload, to the LLM. In most cases, we recommend omitting the task description to avoid unnecessary complications.


\subsection{Examples}

Another optional component for prompts is examples. In theory, providing historical examples can help LLM better understand and handle current task, with the number of examples being   limited only by the token limit of the LLM interface. However, there are several constraints in practical tuning tasks, including (1) database knob tuning tasks often face complex and variable situations, with factors such as workload, queries, database kernel, and hardware differing significantly, which means historical examples might mislead the LLM; (2) high-quality tuning examples are difficult to obtain. Therefore, it is necessary to experimentally test the influence of using examples.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/examples.png}
%     \caption{Relation between examples and tuning results. The  x-axis represents the number of examples in prompt, while the y-axis represents the optimized database performance, represented by QPS.} 
%     \label{fig:examples}
% \end{figure}
\input{tables/prompt_question}

\autoref{tab:prompt_examples} illustrates the relationship between the number of examples and the tuning performance. We found that providing examples can indeed improve LLM's performance in tuning task, but this improvement has its limits. Worse still, when too many examples are provided, the tuning performance actually declines. We believe this is mainly due to the complexity of tuning task. It face highly variable workloads, hardware, and database states, making it difficult to simply learn from other tasks and excessive useless information may interfere with the LLM's judgment.

Further, we also explored the effect of examples' quality. We categorize examples into two groups; those with good tuning performance and similar environment are high-quality examples, and the others are low-quality. As shown in \autoref{tab:prompt_examples}, examples' quality hardly affects LLM tuning results. We believe that the primary value of examples lies in demonstrating the appropriate format for outputting knobs, rather than conveying specific experiential knowledge. Therefore, we recommend providing only one or two examples when tuning with LLM.




==> related.tex <==
\section{RELATED WORK}

We review current approaches for knob tuning and the application
of LLM in database optimization.
\subsection{Large Language Models}
Language Models (LMs) are a fundamental component of natural language processing (NLP) and have been the focus of research for several decades. Large Language Models (LLMs) are a subclass of LMs that leverage massive amounts of data and computational resources to achieve state-of-the-art performance on a wide range of NLP tasks such as machine translation\cite{Aharoni19@LLMtranslate1, Foster18@LLMtranslate2} and summarization\cite{Liu23@LLMsummary1, Sanh22@summary2}. The history of LLMs can be traced back to the early work on neural networks and language modeling. [4] introduced neural language models that learned to predict the next word in a sentence given the previous words. Later, the development of recurrent neural networks (RNNs) and long short-term memory (LSTM) networks further improved the ability of models to capture long-term dependencies in language[22]. However, traditional neural language models still struggled with capturing the rich semantic and contextual relationships present in natural language. The introduction of the Transformer architecture by [52] was a major breakthrough in this area. The Transformer model utilizes self-attention mechanisms to capture the relationships between all elements in a sequence simultaneously, allowing for more comprehensive contextual understanding. This architecture has been used as the backbone of many successful LLMs, including BERT[13], GPT-2[41], and XLNet[60]. ChatGPT[38] is a state-of-the-art dialogue system developed by OpenAI in 2022. It is a state-of-the-art natural language processing (NLP) model that has been widely used in various vertical domains, such as text generation and dialogue systems.

Recently, there has been a lot of research on using LLMs to enhance database systems. DB-GPT [57] introduces an automated prompt strategy utilizing LLMs for query rewriting and index tuning. DB-bert [37] implements the BERT model for database knob
tuning. CodeXDB [36] develops a framework built upon GPT-3 to
simplify complex SQL queries into manageable steps. Additionally,
Trummer [40] offers a tutorial aimed at DBAs on utilizing LLMs
for large-scale data management. Evaporate [1] proposes a com-
prehensive system for processing semi-structured documents into
queryable tables. Furthermore, the capability of GPT to undertake
additional database-related tasks, such as converting text to SQL, is demonstrated in recent works [38, 39]. Although the value of ChatGPT has been validated in various fields, whether it can still be effective in the knob tuning domain remains an under-explored topic, which motivates us to construct such a benchmark to gain insights into the potential of large language models for tuning systems.
\subsection{Database Knob Tuning}
Configuration knobs control many aspects of database systems (e.g., user connections, query optimizer, underlying resource management), and different combinations of knob values significantly affect the system robustness, performance, and resource usage. In general, knob tuning aims to judiciously adjust the values of knobs so as to meet some tuning objectives. For example, the optimizer in relational databases is affected by various knobs like physical operators (e.g., whether allowing to use nested loops in query plans), planning strategies (e.g., heuristic, genetic algorithms), and cost weights (e.g., the cost of random page read). It is vital to set proper values for the knobs in the optimizer so as to generate effective query plans and optimize the performance. Besides, database memory management is also controlled by various configuration knobs, e.g., the space for user connec-tions, the shared buffer size, and the space for background processes. Properly tuning these knobs can avoid frequent disk I/O and improve data access efficiency. Traditionally, knob tuning relies on database administrators (DBAs) to manually try out typical knob combinations, which is highly time-consuming and cannot adapt to a large number of database instances (e.g., tens of thousands of database instances on the cloud). To solve these problems, researchers attempt to design tuning methods that can automatically explore suitable knob settings for different scenarios (e.g., capturing the knob-performance relations with probability models; tuning with the exploration-and-exploitation strategy). 

==> tables/databases.tex <==
% \begin{table}
% \caption{LLM tuning results in different databases.}
% \centering
% \begin{adjustbox}{width=0.48\textwidth}
% \setlength{\tabcolsep}{4pt} % Reduce the space between columns
% \renewcommand{\arraystretch}{1.05} % Adjust the value as needed, 1.5 is 50% larger
% \label{tab:databases}

% \begin{tabular}{cccc}
%     \toprule
%     Database &  Default & LLM & Ratio\\
%     \midrule
%     MySQL & 345 & 2787 & 707.82\%\\
%     PostgreSQL & 417  & 2149 & 415.34\%\\
%     Open Gauss &  432 & 883 & 104.39\%\\
%   \bottomrule
% \end{tabular}

% \end{adjustbox}
% \renewcommand{\arraystretch}{1.0}
% \end{table}


\begin{table}
\caption{LLM tuning results in different databases.}
\centering
\label{tab:databases and benchmark}
\begin{adjustbox}{width=0.48\textwidth}
\setlength{\tabcolsep}{4pt} % Reduce the space between columns
\renewcommand{\arraystretch}{1.05} % Adjust the value as needed, 1.5 is 50% larger

\begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Database} &  \multicolumn{2}{c}{Database Metric} & \multirow{2}{*}{Benchmark} & \multirow{2}{*}{Type} & \multirow{2}{*}{Improvement} \\
    & Release Time & Rank & & & \\
    \midrule
    \multirow{3}{*}{MySQL} & \multirow{3}{*}{1995-05} & \multirow{3}{*}{2} & Sysbench & OLTP & 707.82\% \\
    & & & JOB & OLAP & 87.25\%\\
    & & & TPC-H & OLAP & 91.42\%\\
    \midrule
    \midrule
    
    \multirow{3}{*}{PosetgreSQL} & \multirow{3}{*}{1996-07} & \multirow{3}{*}{4} & Sysbench & OLTP & 415.34\% \\
    & & & JOB & OLAP & 81.76\%\\
    & & & TPC-H & OLAP & 89.89\%\\
    \midrule
    \midrule

    \multirow{3}{*}{TiDB} & \multirow{3}{*}{2017-10} & \multirow{3}{*}{20+} & Sysbench & OLTP & 104.39\% \\
    & & & JOB & OLAP & 74.33\%\\
    & & & TPC-H & OLAP & 80.05\%\\

    \midrule
    \midrule

    \multirow{3}{*}{OpenGauss} & \multirow{3}{*}{2019-05} & \multirow{3}{*}{20+} & Sysbench & OLTP & 107.75\% \\
    & & & JOB & OLAP & 83.74\%\\
    & & & TPC-H & OLAP & 85.91\%\\
    % MySQL & 345 & 2787 & 707.82\%\\
    % PostgreSQL & 417  & 2149 & 415.34\%\\
    % Open Gauss &  432 & 883 & 104.39\%\\
  \bottomrule
\end{tabular}
\end{adjustbox}
\renewcommand{\arraystretch}{1.0}
\end{table}

==> tables/generalization.tex <==
\begin{table*}[t]
\belowrulesep = 0pt
\aboverulesep = 0pt
\caption{Evaluation on Generalization.}
\label{tab:generelization}
\begin{adjustbox}{width=\textwidth}

\begin{tabular}{c|c|cc|cccc|cc}
    \toprule

     \multicolumn{1}{c|}{\multirow{2}{*}{Type}} & \multicolumn{1}{c|}{\multirow{2}{*}{Model}} &  \multicolumn{2}{c|}{Workloads}     & \multicolumn{4}{c|}{Databases} & \multicolumn{2}{c}{Hardware}\\  
      \multicolumn{1}{c|}{} &  \multicolumn{1}{c|}{}                   &  \multicolumn{1}{r}{OLTP($\Delta \% \uparrow$)} & \multicolumn{1}{c|}{OLAP($\Delta \% \uparrow$)}   &  MySQL($\Delta \% \uparrow$) & PostgreSQL($\Delta \% \uparrow$) & TiDB($\Delta \% \uparrow$) & OpenGauss($\Delta \% \uparrow$) & Instance A($\Delta \% \uparrow$) & Instance B($\Delta \% \uparrow$)\\
    \midrule

    \multirow{3}{*}{\makecell[c]{Traditional\\ Method}} 
    & DDPG  & 617 & 204 &  617 & 158 & -32 & \textbf{9} &617 & 126\\
    & SMAC & \textbf{824} & \textbf{270}  & \textbf{824} & \textbf{183} & \textbf{62} & 5 & \textbf{824} & \textbf{169}\\
    & VBO & 812 & 249  & 812 & 171 & 54 & \textbf{9} & 812 & 154\\
    \midrule

    \multirow{4}{*}{\makecell[c]{Closed Source\\ LLM}} & GPT-3.5 &  588 & 242  & 588 & 162 & 10 & 54 & 588 & 158\\
    & GPT-4-Turbo & \textbf{812} & \textbf{303}  & \textbf{812} & \textbf{177} & 56 & 34 & \textbf{812} & 210\\
    & GPT-4o & 641 & 211  & 641 & 173 & 33 & \textbf{62} & 641 & 185\\
    & Claude-3-Opus & 494 & 226 & 494 & 146 & \textbf{60} & 52 & 494 & \textbf{385}\\ 
    \midrule

    \multirow{3}{*}{\makecell[c]{Open Source\\ LLM}} & Llama3-8B-Instruct & 641 & 224  & 641 & 178 & \textbf{35} & \textbf{3} & 641 & 120\\
    & LlaMa3-70B-Instruct & 753 & \textbf{285}  & 753 & \textbf{194} & 30 & -13 & 753 & 104\\
    & Qwen2-7B & \textbf{812} & 264 & \textbf{812} &  131 & 21 & -& \textbf{812} & \textbf{190}\\

    
    

    
    % \multirow{2}{*}{Type} & \multirow{2}{*}{Model} & \multirow{2}{*}{Release Time} & \multirow{2}{*}{Size(B)} & Pretraining Data Scale(tokens) & \\
    % \midrule
    % \multirow{2}{*}{Closed Source} & ChatGPT-3 & 2020.05 & 175 & 300 billion\\
    % & GPT-4 & 2023.03  & - & -\\
    % \midrule
    % \midrule
    % \multirow{2}{*}{Open Source} & T0 &  2021.10 & 11 & -\\
    % & LLaMA &  2023.02 & 65 & 1 trillion\\
  \bottomrule
\end{tabular}
\end{adjustbox}

\renewcommand{\arraystretch}{1.0}
\end{table*}


% \begin{table*}[t]
% \caption{Evaluation on Generalization.}
% \label{tab:knob recommendation}

% \begin{tabular}{cccccccccc}
%     \toprule

%      \multicolumn{1}{c}{\multirow{2}{*}{Type}} & \multicolumn{1}{c}{\multirow{2}{*}{Model}} &  \multicolumn{2}{c}{Workloads}     & \multicolumn{4}{c}{Databases} & \multicolumn{2}{c}{Hardware}\\  
%       \multicolumn{1}{c}{} &  \multicolumn{1}{c}{}                   &  \multicolumn{1}{r}{OLTP} & \multicolumn{1}{c}{OLAP}   &  MySQL & PostgreSQL & TiDB & OpenGauss & Instance A & Instance B\\
%     \midrule

%     \multirow{4}{*}{\makecell[c]{Traditional\\ Method}} & Default & 17 & 2594  & 17 & 52 & 164 & 8.44 & 17 & 500\\
%     & DDPG  & 122 & 853 &  122 & 134 & 110 & 9.17 &122 & 1129\\
%     & SMAC & 157 & 675  & 157 & 147 & 265 & 8.83 & 157 & 1344\\
%     & VBO & 155 & 717  & 155 & 141 & 253 & 9.21 & 155 & 1272\\
%     \midrule
%     \midrule

%     \multirow{4}{*}{\makecell[c]{Closed Source\\ LLM}} & GPT-3.5 &  117 & 758  & 117 & 136 & 180 & 12.98 & 117 & 1288\\
%     & GPT-4-Turbo & \textbf{155} & \textbf{644}  & 155 & 144 & 256 & 11.34 & 155 & 1546\\
%     & GPT-4o & 126 & 833  & 126 & 142 & 218 & 13.69 & 126 & 1462\\
%     & Claude-3-Opus & 101 & 795 & 101 & 128 & 263 & 12.80 & 101 & 2424\\ 
%     \midrule
%     \midrule

%     \multirow{3}{*}{\makecell[c]{Open Source\\ LLM}} & Llama3-8B-Instruct & 126 & 800  & 126 & 144 & 221 & 8.7 & 126 & 1099\\
%     & LlaMa3-70B-Instruct & 145 & \textbf{673}  & 145 & 153 & 213 & 7.35 & 145 & 1021\\
%     & Qwen2-7B & \textbf{155} & \textbf{713} & 155 &  120 & 198 & -& 155 & 1450\\

    
    

    
%     % \multirow{2}{*}{Type} & \multirow{2}{*}{Model} & \multirow{2}{*}{Release Time} & \multirow{2}{*}{Size(B)} & Pretraining Data Scale(tokens) & \\
%     % \midrule
%     % \multirow{2}{*}{Closed Source} & ChatGPT-3 & 2020.05 & 175 & 300 billion\\
%     % & GPT-4 & 2023.03  & - & -\\
%     % \midrule
%     % \midrule
%     % \multirow{2}{*}{Open Source} & T0 &  2021.10 & 11 & -\\
%     % & LLaMA &  2023.02 & 65 & 1 trillion\\
%   \bottomrule
% \end{tabular}

% \renewcommand{\arraystretch}{1.0}
% \end{table*}




==> tables/iteration.tex <==
\begin{table}
\caption{ Tuning effect varies with the number of iterations.}
\centering
\begin{adjustbox}{width=0.48\textwidth}
\setlength{\tabcolsep}{4pt} % Reduce the space between columns
\renewcommand{\arraystretch}{1.05} % Adjust the value as needed, 1.5 is 50% larger
\label{tab:prompt_question}

\begin{tabular}{cccc}
    \toprule
     & Default & Direct Tuning & Incremental Tuning\\
    \midrule
    QPS & 395 &  2787 & 254\\
  \bottomrule
\end{tabular}

\end{adjustbox}
\renewcommand{\arraystretch}{1.0}
\end{table}

==> tables/prompt_input.tex <==
\begin{table}
\caption{Comparison of different input data. "\checkmark"  indicates inclusion in the input, while "\texttimes" indicates exclusion. }
\centering
\begin{adjustbox}{width=0.48\textwidth}
\setlength{\tabcolsep}{4pt} % Reduce the space between columns
\renewcommand{\arraystretch}{1.05} % Adjust the value as needed, 1.5 is 50% larger
\label{tab:prompt_input}

\begin{tabular}{cccc}
    \toprule
    Task Description & Knob Information & Tuning Environment  & QPS\\
    \midrule
    $\times$ &  $\times$ & $\times$ & -\\
    $\checkmark$ &  $\times$ & $\times$ & -\\
    $\times$ &  $\checkmark$ & $\times$ & -\\
    $\times$ &  $\times$ & $\checkmark$ & 2101\\
    $\checkmark$ &  $\times$ & $\checkmark$ & 390\\
    $\checkmark$ &  $\checkmark$ & $\times$ & 1747\\
    $\times$ &  $\checkmark$ & $\checkmark$ & 2833\\
    $\checkmark$ &  $\checkmark$ & $\checkmark$ & 2919\\
  \bottomrule
\end{tabular}

\end{adjustbox}
\renewcommand{\arraystretch}{1.0}
\end{table}

==> tables/prompt_question.tex <==
% \begin{table}
% \caption{Comparison of direct tuning and incremental tuning.}
% \centering
% \begin{adjustbox}{width=0.48\textwidth}
% \setlength{\tabcolsep}{4pt} % Reduce the space between columns
% \renewcommand{\arraystretch}{1.05} % Adjust the value as needed, 1.5 is 50% larger
% \label{tab:prompt_question}

% \begin{tabular}{cccc}
%     \toprule
%     Metric & Default & Direct Tuning & Incremental Tuning\\
%     \midrule
%     QPS & 395 &  2787 & 254\\
%   \bottomrule
% \end{tabular}

% \end{adjustbox}
% \renewcommand{\arraystretch}{1.0}
% \end{table}


\begin{table}
\caption{Relation between the number of examples and tuning results (qps).}
\centering
\label{tab:prompt_examples}
\begin{tabular}{c|c|c|c|c|c}
    \toprule
     & 0 & 1 & 2 & 3 & 4 \\
    \midrule
    high-quality examples & 2252 & 2787 & \textbf{2820} & 2770 & 2739 \\
    low-quality examples & 2252  & 2780 & 2799 & 2781 & 2720 \\
    % \midrule
    % qps & 2252 & 2787 & 2780 & \textbf{2820} & 2799 & 2770 & 2781 &  2739 & 2720 \\
    %QPS & 2252 & 2787 & \textbf{2820} & 2770& 2739 & \\
  \bottomrule
\end{tabular}
\renewcommand{\arraystretch}{1.0}
\end{table}
